Wait or Not to Wait: Evaluating Trade-Offs between Speed and Precision in Blockchain-based Federated Aggregation

This paper presents a fully coupled blockchain-assisted federated learning architecture that effectively eliminates single points of failure by decentralizing both the training and aggregation tasks across all participants. Our proposed system offers a high degree of flexibility, allowing participants to select shared models and customize the aggregation for local needs, thereby optimizing system performance, including accurate inference results. Notably, the integration of blockchain technology in our work is to promote a trustless environment, ensuring transparency and non-repudiation among participants when abnormalities are detected. To validate the effectiveness, we conducted real-world federated learning deployments on a private Ethereum platform, using two different models, ranging from simple to complex neural networks. The experimental results indicate comparable inference accuracy between centralized and decentralized federated learning settings. Furthermore, our findings indicate that asynchronous aggregation is a feasible option for simple learning models. However, complex learning models require greater training model involvement in the aggregation to achieve high model quality, instead of asynchronous aggregation. With the implementation of asynchronous aggregation and the flexibility to select models, participants anticipate decreased aggregation time in each communication round, while experiencing minimal accuracy trade-off.

==> txt/Background-old.tex <==
\section{Background} \label{sec:technologies}

    \subsection{Federated Learning}
    %\todo[inline]{Huong: write some more concept related to federated learning, why its better to train in this decentralized way}
    
    FL is a way of setting a training model in a collaborative and decentralized way, where no one's data can be seen or touched by others in the learning process. The setting was born based on the principles of mitigating the shortcomings of traditional centralized training, particularly user privacy risks and large datasets required \cite{kairouz2021}. The main goal of the ``federated'' is to ensure that we get the high accuracy of the centralized model at the end while still keeping the training data distributed and stored at the clients' sides.
    
    % how it work
    It can be easy to point out the advantages of the FL against the traditional method when we look at how they work. Contrary to the traditional way of training a model, where a huge amount of data needs to be sent to a central server to process and train, which may cause bottlenecks and heavy traffic to the central cloud, here, under FL, multiple participants can remotely contribute their works to build a single global model. Each party in the network downloads the same initial model from the server to start the training process with a loop of repeated steps in the order: local train, upload to the server, download the aggregated model, and continue the local training. To be more specific, the local model will be trained only on the private data of the party, and then model configurations will be encrypted before sending to the central aggregator to decrypt, and calculate the average for the global model. The Federated Averaging (FedAvg) algorithm that works in FL is presented in pseudocode as Algorithm \ref{algo:fedavg}.
    
    \begin{algorithm}[]
    \DontPrintSemicolon
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Initialization}{Initialization}
    \SetKwFor{For}{for}{do}{end for}
    \SetKwFor{ForEach}{foreach}{do}{end foreach}
    \SetKwIF{If}{ElseIf}{Else}{if}{then}{else if}{else}{endif}
    
    \caption{FedAvg}
    \label{algo:fedavg}
    \Input{$N$ total number of clients \\ $\mathbb{R}$ number of communication round \\ $\mathbb{E}$ number of training epochs \\ $P_k$ set of data at client $k$\\ $\eta$ learning rate \\ $\nabla(w, b)$ w's gradient on batch $b$}

    \tcp{AGGREGATOR SIDE}
    
    \Initialization{initialize $w_0$}
    \For{$t$ from $1$ to $\mathbb{R}$}{
        $\mathbb{K} \gets$ set of selected $M$ clients $ (M \leq N)$\;
        \ForEach{client $k \in \mathbb{K}$}{
            $w_{t+1}^k \gets \text{LocalTraining}(k, w_t)$\;
        }
        $w_{t+1} \gets \frac{1}{M}\sum_{k=1}^M w_{t+1}^k$\;
    }
    
    \tcp{CLIENT SIDE}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\textup{LocalTraining}$(k, w)$}{
        \For{$e$ from $1$ to $\mathbb{E}$}{
            $\mathbb{B} \gets$ data batches split from $P_k$ by pre-set batch size\;
            \ForEach{batch $b \in \mathbb{B}$}{
                $w \gets w - \eta \nabla(w; b)$\;
            }
        }
        \KwRet{$w$}
    }
\end{algorithm}

    
    % types of FL
    % The FL comes in three forms, where each is defined by how the data is split: horizontal, vertical, and transfer. 
    
    % \textbf{Horizontal FL (or sample-based FL):} in this type of learning, models are trained on similar datasets, where samples from different devices across the network have the same set of features \cite{yang2019fed}. For example, in the human detection task, we have to build separate models from different continents and then combine them into one global model. As a matter of fact, we can easily see the differences between Africans and Asian or European citizens based on skin colour, physical body, etc. However, people from different geographical locations are still the same species and have many things in common such as body parts so that the feature space can be the same (E.g. hair colour, lip thickness, nose height, ear shape, height, weight, and more).

    % \textbf{Vertical FL (or feature-based FL):} \cite{wei2022vert} uses different datasets in a complementary way, where they share the same object's identity but differ in feature sets. An applicable example could be a collaboration among companies. In particular, assuming that a technology company has owned the user's web surfing data and a specific bank owns the user's purchasing transactions. In this case, obviously, these two data have no common feature spaces. However, we still can utilize the collaborative data from both parties to jointly train a model to suggest better advertisements in the next web browsing. 

    % \textbf{Federated Transfer Learning:} \cite{LiuKXCY20, chen2020fedhealth} this type of learning is applicable in scenarios where datasets differ in both horizontal and vertical ways. With the concept of transfer learning, a pre-trained model, which is designed to perform one specific task, will be fine-tuned and personalized to solve a related or similar problem on a different dataset (e.g. a pre-trained model on a cat dataset can be used to fine-tune for bird detection). From a practical perspective, different parties in the federated learning system may have a specific feature space for themselves; however, they still want to leverage the collaboration with others in the network to solve their problem, especially when they do not have a sufficient amount of data to train their own model \cite{saha2021federated}. By employing a few common sample sets, a synthetic representation of two feature spaces will be learned, which is then applied to get predictions for samples with only one-side features (only contains one feature space). That is how Transfer Learning meets the Federated system.

    % why its better than traditional way / pros
    In the end, this emerging learning method has raised a question about ``why we use FL instead of learning in the traditional way?''.  This can be explained by the benefits it gains from how it works in a decentralization and cooperation way. To be more specific, the use of distributed datasets over parties helps avoid data centralization with high latency and no privacy. In this way, FL also gives parties better control over how their personal data is processed. Regarding privacy issues, decentralization in FL minimizes the amount of private data to be transferred and processed by a third party throughout the training process. Finally, when the contributions to the ``commonwealth'' of the whole organization or higher-authorized area are expected to be anonymous, FL becomes the best fit since it facilitates training the model with data from ``nameless'' users. 
    
    % drawbacks / cons
    Beyond the foregoing, the FL framework still has many drawbacks related to model performance, communication issues, and vulnerabilities. As a matter of fact, there is always a trade-off between efficiency and privacy in FL. From that, in order to boost privacy protection, noise is usually added to data, which coincidentally causes accuracy loss. However, regarding this, FL decides to sacrifice the performance of the model by adding the noise, but at a compromise amount. Next, communication cost is another concern in FL, especially when there are millions of connected devices in the network. The bottleneck at the aggregator is dangerous for the whole system as it can stall the learning process and cripple some training devices while it cannot transfer and update the models on time.

    % \subsection{Threat models and adversarial attacks}
    % \todo[inline]{not really need this.....i guess}
    % \label{sec:threat-model}
    % poisoning attack
    % inference attack
    % In general, there are two main attacks on an FL system, which aim at data privacy and model qualitỵ
    % In particular, data poisoning is related to the possibility of reconstructing the raw data from shared parameters (reconstruction attack) [3, 4, 5] and the inference of the origin of the data record if it was included in or belong to the local training dataset (member reasoning attack) [6, 7]. Model poisoning attacks, on the other hand, focus on affecting the quality of the model, including the untargeted attack to decrease the accuracy of the global model on all classes [8] and the targeted attack at specific classes with label flipping and backdoor attack techniques [9, 10]. Based on that, secure, private, and fast aggregation in a large-scale FL system is getting more attractive to researchers nowadays [11, 12]. 
    % \subsubsection{Data poisoning} 
    % \begin{itemize}
    %     % \item dirty-label attack 
    %     % \item clean-label attack 
    %     % https://proceedings.neurips.cc/paper/2018/file/22722a343513ed45f14905eb07621686-Paper.pdf
    %     \item member reasoning attack
    %     \item reconstruction attack
    % \end{itemize}
    
    
    % \subsubsection{Model poisoning: }
    % \begin{itemize}
    %     \item label-flipping
    %     \item backdoor 
    % \end{itemize}
    
    
    
    % https://arxiv.org/pdf/2201.08135.pdf
    
    % https://arxiv.org/pdf/2003.02133.pdf *** \cite{Lyu_2020}
    
    % % \subsection{Fully Decentralized Federated Learning}
    % %     \cite{lalitha2018fully}
        
    % %     http://bayesiandeeplearning.org/2018/papers/140.pdf
        
    % %     https://arxiv.org/pdf/1901.11173.pdf
    \subsection{Blockchain technology}
    %\todo[inline]{Tri: write the concept, base structure, principle works, why it can be used in many disciplines}
    
    % concept, 
    Blockchain technology is a public database deployed in a decentralized environment from an array of participants. After the first introduction of cryptocurrencies, blockchain has been utilized in different fields due to the immutability feature and consensus mechanism. Unlike centralized systems, deploying a system in a decentralized area strictly demands a unique state from different participants. Thus, immutability is the prime characteristic of the success of the decentralized system. Blockchain technology especially separates the system's timeline into consensus rounds or epochs every ten minutes or after limited operations. At each round, a consensus has to finish deciding and wrapping a chronological order of transactions into a block. The immutability of blockchain is from hashing schemes, by which each new block calculates and stores a hash value of the previous. Meanwhile, another crucial part is about the consensus mechanism to select transactions or well-behaviour participants as a leader to obey the protocol without conflict between transactions. %Therefore, a blockchain-based system succeeds in a decentralized environment via the immutability and 
    
    Although the success of blockchain encourages centralized systems to transform into a decentralized environment, leveraging blockchain technology requires flexibility; hence, blockchain-based smart contracts such as Ethereum~\cite{wood2014ethereum,buterin2014next} is the key evolution that current systems desire to utilize. Recognizing the lack of Turing completeness from previous blockchain-based systems, Buterin et al. propose one of the first blockchain-based smart contract platforms that allow distribution system operations among participants. Therefore, the system's participants have the same view based on the blockchain's characteristics. Regarding this deliberation, other studies adopt the blockchain-based smart contract concept as the next-generation communication with decentralization and flexibility, especially single-fault tolerance.
    
    Due to its accessibility, blockchain technology is categorized into two main perspectives: permissioned and permissionless. Permissioned blockchain is considered a private system in a decentralized environment, which requires each participant to own a unique identity. Meanwhile, the other allows freedom in data accessibility. Therefore, the permissioned blockchain supports authorization and authentication but impacts flexibility and privacy considerations. Instead, the permissionless blockchain provides flexibility for network accessibility and is hard to privacy track. However, from the performance perspective, the permissioned blockchain platforms dominate the permissionless platforms~\cite{NGUYEN2023606} due to the security requirement of leader selection in consensus rounds, for example, Proof-of-Work  as Bitcoin and Ethereum.

    % \begin{figure}
    %     \centering
    %     \includegraphics{}
    %     \caption{Blockchain structure }
    %     \label{fig:blockchainStruture}
    % \end{figure}
    

    \subsection{Blockchain-based Federated Learning}
    %\todo[inline]{Tri}
        Leveraging blockchain technology evolves in different perspectives, especially architecture for various decentralized types; however, the deployment of blockchain requires an analysis for promising adaptions. 
        
        \subsubsection{Architecture toward Decentralization}
        % architecture
        One of the interesting considerations is the harmonization of architecture between FL and blockchain architecture. In detail, initial FL is introduced with a mater-slave architecture, while decentralization is the foundation of blockchain technology. Regarding a survey work from Wang et al.~\cite{wang_2021}, the current works of FL leveraging the blockchain in three directions from the architecture perspective. The first view of blockchain-based FL is about \textbf{fully coupled}, which points to the FL clients handling blockchain tasks. \textbf{Semi-coupled} blockchain-based FL is about the deployment of blockchain tasks from the FL aggregator via many participants. Finally, \textbf{loosely coupled} between blockchain and FL is a concept in which the blockchain provides services, for example, access management or reputation for enhancing FL features, especially from a security viewpoint. 
        
        %\subsubsection{Benefits}
         % Enhancement of features
        Despite the various architectures from the combination of blockchain and FL, a fully coupled integration is the most attractive in a decentralized setup. In detail, a fully coupled blockchain-based FL system transforms traditional FL into a decentralized environment when local devices need to train local data and deploy blockchain tasks, including block formation, propagation, and verification. Hence, each system's local device requires many resources for the storage and computation of both tasks. However, another benefit of a fully coupled blockchain-based FL is the capability to deploy various services like other combinations between blockchain and FL via the smart contract concept.
        
        Semi-coupled and loosely coupled combinations of blockchain and FL do not support a decentralized when the blockchain tasks and FL tasks disjoint partially or totally. Therefore, the main issue related to single-point failure remains, and the complexity of the intersection of two systems raises challenges in management. Despite drawbacks, these deliberations aim to enhance the system's performance from communication and computation but still adopt secure features from blockchain technology, for example, reputation management or incentive strategy, to avoid free-rider issues. Regarding these perspectives, this study prefers to emphasize fully coupling blockchain and FL for the single-point-failure feature.
        
       % Since leveraging blockchain enables consistent data sharing among participants in a decentralized network, FL, a slave master architecture, adopts blockchain technology 
        
        \subsubsection{Services and Usages}      
        % Blockchain stores model or how current work 
        %The traditional FL does not mention the viewpoint in 
        Due to the lack of honest workflow and reliable data in FL, blockchain supports FL in local model verification, global aggregation, and information storage.

        Model verification aims to reduce the disobedience from uploaded local models to avoid intentional or unintentional noise. A blockchain protocol for model verification can be from a consensus mechanism like~\cite{kang_2020, Li_2021} with Proof-of-Verifying. This concept utilizes a reliable testing dataset to evaluate uploaded models. In detail, an idea utilizes a consensus to ensure and select suitable local updates; however, the system requires defining a suitable verification approach to filter noise-uploaded models. Similar to this consideration is a reputation-based system, which utilizes a history of feedback to evaluate the trustworthiness of up-loaders.

        %Aggregation of global model
        The aggregation for the global model is from several selected blockchain participants or all participants. The main difference between those is about the resources requirement according to tasks. In other words, this perspective is similar to a consensus mechanism to arrange agreements among participants and ensure security. In detail, the selected blockchain participants are representatives to contribute and verify system decisions as global aggregation. Thus, the efficient communication and computation performance is better than the aggregation from all participants. Meanwhile, when all participants aggregate the global model, each participant needs the exchange and storage of local models. Hence, the performance is a barrier to developing the system; however, the trust or approaches for selective representers can be flexible.
        
        
        %Data storage of a blockchain-based Federated Learning
        Blockchain-based FL introduces secure data storage and exchange via an open environment. Due to the benefits of blockchain technology, blockchain-based FL provides immutability and audit to exchange uploaded models and global models via cryptographic schemes and consensus mechanisms from the blockchain. Therefore, confirmed models stored in the blockchain are guaranteed from late modification, which is also a piece of evidence for non-repudiation to detect abnormality.

        
        %\subsubsection{Blockchain-based Federated Learning for Applications}
        
